How Does Generative Retrieval Scale to Millions of Passages?

Popularized by the Differentiable Search Index, the emerging paradigm of generative retrieval re-frames the classic information retrieval problem into a sequence-to-sequence modeling task, forgoing external indices and encoding an entire document corpus within a single Transformer. Although many different approaches have been proposed to improve the effectiveness of generative retrieval, they have only been evaluated on document corpora on the order of 100k in size. We conduct the first empirical study of generative retrieval techniques across various corpus scales, ultimately scaling up to the entire MS MARCO passage ranking task with a corpus of 8.8M passages and evaluating model sizes up to 11B parameters. We uncover several findings about scaling generative retrieval to millions of passages; notably, the central importance of using synthetic queries as document representations during indexing, the ineffectiveness of existing proposed architecture modifications when accounting for compute cost, and the limits of naively scaling model parameters with respect to retrieval performance. While we find that generative retrieval is competitive with state-of-the-art dual encoders on small corpora, scaling to millions of passages remains an important and unsolved challenge. We believe these findings will be valuable for the community to clarify the current state of generative retrieval, highlight the unique challenges, and inspire new research directions.

==> experiments_backup.tex <==
\section{Experimental Setting}\label{sec.setting}
\subsection{Datasets}\label{subsec.datasets}
We begin with small-scale experimentation matching the setting posed by~\citet{Wang2022ANC} to accurately reproduce their findings.
That is, we use the Natural Questions~\cite{kwiatkowski2019natural} and TriviaQA~\cite{joshi2017triviaqa} datasets processed and provided in the NCI codebase.
More specifically, we use the documents, the segmented documents, the training/testing sets and the generated queries from their repository but generate our own semantic identifiers as we diverge slightly in its creation methodology.

The Natural Questions and TriviaQA datasets have corpora of sizes $109$K and $74$K, respectively.
As mentioned earlier, each of them also has roughly 20 and 15 generated queries for every document.
Their training generation tasks have $307$K and $111$K query examples, each.

To advocate a switch to standard relevance ranking datasets, we also propose using the MS MARCO passage ranking task to see if the findings are consistent.
The full MS MARCO passage ranking datasets has a corpus of 8.8M passages and a training set of 532K queries but to build up to this scale we suggest three incremental variants:
\begin{itemize}
    \item MS-100K - Similar to~\citet{Zhuang2022BridgingTG}, we curate a dataset which focuses on only 100K passages of the corpus and all questions corresponding to those passages.
    However, it is worth noting that the sampled set is distinct from theirs, so a one-to-one comparison in effectiveness does not hold ground.
    We ensure that the passages selected in all variants cover the development set (which is consistent across the variants) and every other passage not covered by the development set is covered by the training set of queries.
    This corpus size is comparable to those of the datasets explored in the Neural Corpus Indexer.
    \item MS-1M - We introduce this setting as it indicates a $10 \times$ scale up in the corpus size.
    Here, roughly $50\%$ of the passages do not have a question in the training set, which diverges from all our smaller scale datasets.
    \item MS-Full - Here, we yet again see another order of magnitude scale up in corpus size.
    As a result, only $6\%$ of the passages have a corresponding query in the training set.
    Having a model that indexes a corpus of this size in its model parameters forms an interesting experiment that has never previously been done in the literature.
\end{itemize}

We incorporate all the datasets mentioned into $\texttt{t5x}$, a framework capable of creating scalable data pipelines that feed into our downstream sequential models.
For the Natural Questions and TriviaQA datasets, we create tasks to capture the indexing the whole Wikipedia document as well as the Document As Query setting.
We also add generation tasks for the training query set, the doc2query--T5\textsubscript{MARCO} generated query set and the doc2query--T5\textsubscript{InDomain} generated query set. 

Given these tasks, various mixtures are considered which sample across the tasks during training with equal probability.
More specifically, we consider the NCI\textsubscript{daq}, NCI\textsubscript{daq+gen}, NCI\textsubscript{daq+gen+d2q}, \\ NCI\textsubscript{daq+gen+d2q+idx}, and NCI\textsubscript{daq+gen+d2q+idx+d2qid} settings, each representing the incremental addition of the Document As Query set, training query set, doc2query--T5\textsubscript{MARCO} generated query set, whole Wikipedia document set, and doc2query--T5\textsubscript{InDomain} generated query set, respectively.
This helps us determine which of these tasks are crucial to the end-to-end effectiveness in our ground up study.

For the three MS MARCO variants, we first create a task to facilitate the indexing of the passages (idx) but do not include the Document As Query setting, given that it does not make sense in the passage ranking setting to consider segments of the passage.
We add generation tasks for the training query set (gen) and the different doc2query--T5\textsubscript{MARCO} generated query sets considered (d2q).

As we scale to full MS MARCO passage ranking task, we believe that the exposing the model to the indexing and generation task (of only the training set queries) with equal probability leads to an overexposure of the training query set given that there are only 500K queries and 8.8M passages.
Hence, we find that sampling the query once for every time we sample 32 passages works best and the mixture NCI\textsubscript{idx+gen} implicitly indicates this sampling ratio for the MS-Full setting.

In all our tasks and mixtures, we ensure that all the text is pre-processed to be lowercase.
\subsection{Metrics}\label{subsec.metrics}
For the NQ and TriviaQA experiments, we match the primary metric followed by the Neural Corpus Indexer and DSI, Hit@$N$.
Based on their experimental table, they have Hits@1 as the primary metric for Natural Questions and Hits@5 as that for TriviaQA

For the MS MARCO passage ranking variants considered, following the literature, we focus on Mean Reciprocal Rank at 10 (MRR@10) as our primary metric.
\subsection{Baselines}\label{subsec.baselines}
Our first baseline is the traditional BM25 algorithm.
We leverage the Pyserini implementation~\cite{Lin_etal_SIGIR2021_Pyserini} of BM25 with default hyperparameters. 

Our second baseline is the BM25 (w/ doc2query--T5), as explored in~\citet{nogueira2019docT5query}.
This has been shown to be an effective first stage retrieval method in prior work.

For the NQ and TriviaQA datasets, we compare our models to the scores of the best reported T5-base model in NCI and their reproduction of DSI.

For the MS MARCO passage ranking variants, we compare the models to GTR-base, a strong dense retriever.
While GTR leverages a variety of other techniques and advancements in bi-encoder literature to achieve state-of-the-art effectiveness for dense retrievers, we include these results as a sort of goal post of what a true Neural Corpus Indexer should be capable of.
It is worth noting that such dense retrievers offload dense encodings for each passage (for a corpus of 8.8M passages, this is roughly 7 billion parameters offloaded), so they do not worry about capturing all passage information within the model parameters, something the Neural Corpus Indexer has to achieve with its limited T5-base architecture (220 million parameters).


\subsection{Implementation Details}
Our replication of Neural Corpus Indexer leverages \texttt{t5x}~\cite{roberts2022t5x}, a composable and research-friendly framework for large scale training and evaluation of sequence-to-sequence models.
This framework relies heavily on JAX, Flaxformer and Flax libraries.
Meanwhile the original NCI codebase was built on the HuggingFace library.

We initialize our models with the pretrained T5-base model and in the case that we use the PAWA decoder, we randomly initialize the PAWA model parameters.
For the MS MARCO variants, we set the maximum input sequence length to be 128 for all experiments, while for the NQ and TriviaQA tasks this was set to 64, matching the NCI setup.
The batch size in all our experiments is set to 512 as we generally note that larger batch sizes lead to more stable training.
We train our models with a learning rate of $1 \cdot 10^{-3}$ and a droupout rate of $0.1$.

We find it enough to train the small-scale experiments for 1M steps but when we scale our models to the larger corpora, we need to train our model for 9M steps before it converges in certain settings, especially when we use sequential document identifier.
As a result, the training with these settings takes about ten days as opposed to a day in the regular settings on Google's TPU v4-8s.

==> extensions_analysis_backup.tex <==
\section{Our Extension}
In this section, we explore some other questions we believe are fundamental to better understanding the effect of query generation, which seems to be a crucial component in building Neural Corpus Indexers.
\subsection{Effect of In-Domain Query Generation}
For the Natural Questions and TriviaQA datasets, using the query generation model, doc2query--T5\textsubscript{MARCO} trained only on the MS MARCO passage ranking task is likely sub-optimal.
This is because the average MS MARCO passage, which is extracted from search engine results, varies drastically from the average Wikipedia article.
To this end, we propose training an in-domain query generation model on the Natural Questions dataset.

[insert details Kai].
% \subsection{Effect of filtering Generated Query Sets}
% We follow some recent advancements in utilizing neural cross encoders to refine the generated query set of incoherent, unspecific queries, as seen in~\citet{d2q-less-more}.
% More specifically, we leverage a RankT5-XL model to first score (generated query, passage) pairs and then filter out those generated queries that give a low ranking score.
% The threshold is such that we filter out $x\%$ of the queries to make the query set more relevant, coherent and hallucination-free.
% This can be considered both as a global threshold, as in we filter out $x\%$ of all queries in the generated query set or a local threshold where we filter out $x\%$ of queries belonging to a particular identifier.

% \input{tab_d2q_rankt5}

%TODO
\subsection{Different DocIDs}

% In table
\subsection{Dependence on number of queries, temperature, and top-$k$ decoding}
In this experiment, we try to discern the importance of different factors of the synthesis of the doc2query--T5 query set that impact its NCI generation task.
To this end, we first train our own doc2query--T5\textsubscript{MARCO} model and use it to generate queries for the MS-100K subset.

Given this trained model, while running query generation, we can vary certain hyperparameters which we believe critical to understanding the effect of query generation --- the $k$ in top-$k$ sampling (10 vs.\ 20), the number of generated queries (40 vs.\ 100), the temperature (1.0 vs.\ 0.7) and the filtering out synthetic queries having fewer than 4 words.
This filtering is motivated by the fact that queries with fewer than four words are likely incoherent or lack specificity. 

\input{tab_d2q_count}
Table~\ref{table:v1:passage_n_queries} denotes the results of all these ablations.

Firstly, comparing rows ($\ast$a) and ($\ast$b), it is clear that the length filter seems slightly detrimental to the effectiveness of NCI\textsubscript{d2q}.
We are also able to closely reproduce the results when using the original synthetic query set provided by~\citet{Ma2022DocumentEB}, as can be seen comparing row (1b) with the effectiveness to the atomic setting in row (2d) of Table~\ref{table:v1:passage_subset}, both of which result in an MRR@10 of $80.3$.

Increasing the number of queries generated to $100$ seems to have a big boost in effectiveness, as can be seen comparing rows (2$\ast$) with rows (1$\ast$).
The improvement makes sense as the neural corpus indexer is introduced to more unique queries likely answered by the passage as we generate more synthetic queries thereby resulting in higher development set effectiveness.
This helps bridge some of the gap between the NCI\textsubscript{d2q}
 and the powerful dual encoder, GTR-base (Table~\ref{table:v1:passage_subset}, Row (1c)).

Since decreasing the decoding temperature increases the probability of more likely tokens and sequences, it is expected that the diversity in the synthetic query set suffers if the temperature is reduced.
As seen comparing rows (1$\ast$) and (3$\ast$), we note that this drop in diversity, results in a drop in effectiveness.

Decoding with top-$k$ sampling and higher values of $k$, increases the shortlist the model will sample from and as a result would improve the diversity in the synthetic query set.
As we note in rows (4$\ast$), the result is a slight improvement in effectiveness, albeit likely not significant.

More analysis of the diversity and amount of queries considered to peek out the effectiveness of these neural corpus indexers are required and likely at different corpus scales.


==> introduction_old.tex <==
\section{Introduction}\label{sec.intro}
Information Retrieval has been an active area of research for several decades and has seen remarkable progress in various applications for tasks such as search, recommendations, and question answering.
However, most of this progress in this age of transformers~\cite{vaswani2017attention} and large language models lies in the ``retrieve--then--rank'' paradigm.
\citet{metzler21rethinking} envisions modeling in the ``unified retrieve--and--rank'' paradigm, which we dub Unified Generative Retrievers. Herein, the entire indexing, retrieval, and ranking components of the traditional multi-stage ranking pipeline is integrated into a single consolidated sequence-to-sequence model, where indexing is replaced by model training, and retrieval and ranking are replaced by model inference.
That is, the model, would form the index in itself, capable of mapping input queries directly to document identifiers. Such a reformulation converts the ranking tasks into seq2seq task~\cite{2020t5}, making it align better with the other natural language generation tasks. 

The Differentiable Search Index~\cite{Tay2022TransformerMA} is the first realization of this goal, where a T5-style encoder-decoder model~\cite{2020t5} was used to model the mapping of queries to relevant document identifiers.
The models were co-trained on the indexing task, where the goal is to memorize information about each document and the retrieval or generation tasks where the model learns to effectively retrieve from the model parameters.
% Three kinds of document identifiers were considered --- the atomic identifier, where a single token is decoded corresponding to the document identifier, the naive string identifier, where a random string of tokens is to be decoded, and the semantic string identifier, where a string is first pre-computed for each document capturing some notions of a semantic hierarchy and the model is to decode such identifiers.
% However, the model is evaluated on a small-scale question answering dataset, Natural Questions and while indexing, the model is exposed to only the first 64 tokens of the document.

Neural Corpus Indexer (NCI)~\cite{Wang2022ANC} follows DSI and introduces a few components to further boost end-to-end effectiveness.
On top of DSI, several components are  experimented with,
including the addition of the ``document as query'' (DaQ) task,
question generation (D2Q) task,
Prefix-Aware Weight-Adaptive (PAWA) Decoding on top of Hierarchy-Aware Semantic Identifiers, Constrained Decoding, and Consistency Regularization Losses.
These components are summarised and introduced in detail in Table~\ref{tab.method} and 
Section~\ref{sec.methods}, respectively.

Both DSI and NCI evaluate their results on small scale question answering datasets --- Natural Questions (NQ)~\cite{kwiatkowski2019natural} and TriviaQA~\cite{joshi2017triviaqa}.
These datasets have around 100K documents in the corpus.
While such an evaluation setup serves good for a proof of concept,
it falls short of the scale in widely accepted ranking benchmarks.
Besides, almost all documents in these corpus have corresponding queries in the training set,
thereby not subjecting their models to ``true generalization'' to most passages without any training queries, which is the norm with \emph{ad-hoc} retrieval.

In light of the importance of unified generative retrieval problem, 
we begin with a replication study of the Neural Corpus Indexer~\cite{Wang2022ANC}, where we evaluate the effectiveness of NCI on the Natural Questions and TriviaQA datasets processed and provided by the authors.
We do so building our own codebase from scratch, with heavy integration of the \texttt{t5x} toolkit~\cite{roberts2022t5x}, a composable framework useful for large scale training of language models.
% , an aspect important to our study.
% Tasks are incrementally added to our final mixture to determine which components are vital to model effectiveness.
    % Similarly, different model components are ablated to determine the vitality to the final Neural Corpus Indexer model in our setup.

Given successful reproduction, we switch gears to the widely-used MS MARCO Passage Ranking task, beginning with a 100K passage subset.
% , following a curation similar to~\citet{zhuang2022bridging}.
Afterwards, we scale up incrementally to a 1M subset followed by the full task with 8.8M passages.
This final corpus is about $90 \times$ larger than those considered in other studies, making it an important landmark for the community.
    % Here too, we note trends with different representations of document identifiers.

To this end, we answer following research questions: 
\newline\paragraph{(RQ1) Can we replicate the NCI results and which of its components are necessary for its success?}
\newline\paragraph{(RQ2) How does NCI perform at large scale, on the two variants of the MS MARCO Passage Ranking dataset with 1M and 8.8M passages?}

\noindent And finally, we attempt to answer the question posed in the title: \newline\paragraph{(RQ3) What makes a unified generative retriever work?}

Through extensive experimental studies, 
we find that leveraging synthetic queries from question generation (D2Q) is the single crucial component that contributes to the effectiveness of the model; and show that in-domain generated queries as well as increasing the diversity in the synthetic query pool could bring in further performance boost.
Ultimately,
putting all the findings together, we demonstrate a model, coined as UGR, that exploits useful components from DSI and NCI. 

The contributions of this paper are threefold. (1)
To the best of our knowledge, this is the first experimental study to rigorously examine UGR models
on widely-used ranking benchmarks; (2)
Through ablation study, we examine  
different design choices and model components, enlightening future studies in this direction; (3) Our UGR model advances the effectiveness on top of DSI and NCI, laying a strong foundation for  future work in this field.





% We further investigate the role of query generation, which we find to be one of the keys to this puzzle of building scalable unified generative retrievers.
%     We find that in-domain generated queries as well as increasing the diversity in the synthetic query pool are two important aspects to the success of Unified Generative Retrievers.
% \end{itemize}

==> method_backup.tex <==
\section{Methods}\label{sec.methods}

In this section, we begin with a description of Neural Corpus Indexer (NCI)~\cite{Wang2022ANC}, a sequence-to-sequence language model capable of mapping string queries directly to relevant document identifiers (DocIDs).
To build to this model, we begin with its core backbone, the Differentiable Search Index (DSI)~\cite{Tay2022TransformerMA} and explore the different document identifier representation stategies, going beyond those considered by~\citet{Wang2022ANC}.

Then, we go over the critical aspects of the Neural Corpus Indexer that differentiate it from DSI.
We begin with their proposed Document As Query (DAQ) technique, where randomly chunked segments of the documents are exposed to the model during training. 
It alleviates issues stemming from documents being too long for transformers to process in a single pass because of computational constraints.

Next, we look into how to leverage synthetic queries to alleviate some drift between the training and target evaluation task, given most passages in large corpora do not have corresponding training queries, especially in larger corpora.
Here, we also investigate the importance of in-domain query generation and how filtering out incoherent, less relevant synthetic queries can play a role in improving the effectiveness of our trained models.

We then investigate the effectiveness brought about by the Prefix-Aware Weight-Adaptive Decoder, a key architectural distinction leveraged by~\citet{Wang2022ANC}.
Next, we describe constrained decoding, a method to dissuade the decoding of identifiers not corresponding to the corpus.
Finally, we describe their proposed consistency loss, which serves as a regularization method for the Neural Corpus Indexer.
% Finally, we go over two schemes that incorporate negative samples in training the generation of DocID from the queries, an aspect ignored by previous studies.
% This is done on the loss level by incorporating the unlikelihood loss and the length-normalized loss, a generalization of the learning-to-rank SoftMax loss to sequence-level targets.
% On the prompt level, we analyze if providing DSI with a list of DocIDs can aid the model make higher order comparisons between them to aid in end-to-end effectiveness.

\subsection{Neural Corpus Indexer}
The core principle governing Neural Corpus Indexer is to fully parameterize a traditional neural retrieval pipelines within a single sequence-to-sequence model.
This is heavily inspired by Differentiable Search Index (DSI)~\cite{Tay2022TransformerMA}.
Since the model is a generative retrieval model, trained to generate the document identifiers (DocIDs) in all tasks, the output is always the textual string corresponding to that document identifier.
To achieve this, they proposed two core training tasks:
\begin{itemize}
    \item \textbf{Indexing Task (idx):} Models the mapping of each document $d_i$ to the textual representation of its corresponding identifier $i$.
    More specifically, the following input template is passed onto the model:
\begin{equation*}
    indexing: \ \ d_i
\end{equation*}
    \item \textbf{Generation Task (gen):} Models the mapping of a given query $q$ to the textual representation of its corresponding identifier $i$.
    More specifically, the following input template is used:
\begin{equation*}
    generation: \ \ q
\end{equation*}
\end{itemize}

Given that the goal is to build a retrieval system capable of retrieving documents corresponding to user queries, the generation task represents the target task we are trying to explicitly model.
During inference, the NCI/DSI model returns a ranked list of candidate DocIDs leveraging beam search.

The next subsection looks into the different approaches explored in this paper with respect to the modeling of the target space, i.e., the document identifiesr.

\subsubsection{DocID Representation Strategies}
Taking cues from Differentiable Search Index~\cite{Tay2022TransformerMA} as well as Neural Corpus Indexer~\cite{Wang2022ANC}, we explore the following strategies of modeling the document identifiers.
\begin{itemize}
    \item \textbf{Atomic DocID:} In this setting, models are trained to emit one logit for each unique DocID.
    This is done by augmenting the vocabulary space with $|C|$ new tokens, each corresponding to a document identifier.
    In this case, the output target sequence is always a single token in length, hence the ``atomic''.
    
    With each of these new tokens comes the introduction of $|C|$ corresponding token embeddings, each of which is randomly initialized during model training.
    Note that doing this results in a blow-up of model parameters, given the linear dependence on $|C|$ which in our settings can often be in the order of millions.
    Hence, we should be careful while making comparisons with other representation stategies.
    \item \textbf{Naive DocID:} In this setting, models are trained to generate the textual string ``\emph{[doc\_{id}]}'', where \emph{id} is the original document identifier in the corpus.
    We consider this a sequential setting and the model generates the target using the original input vocabulary of T5, our base model.
    During inference, beam search is used to obtain a ranked list of document identifiers.
    Our beam size across all experiments is $b = 100$ and the target token size either $8$ or $16$ depending on the dataset considered.
    It is worth noting that such naive document identifiers might already capture some semantics of the corpus, as it is dependent on the curation pipeline, but the semantics captured if any are likely not rich.
    \item \textbf{Semantic DocID:} In this setting, following the NCI terminology, models are trained to generate the textual string ``\emph{id}'', where \emph{id} is a semantic document identifier generated for each document in the corpus.
    This method borrows a lot of key ideas from DSI.
    The method relies on two core components -- using a language model to first generate an encoding of the text and a hierarchical $k$-means clustering algorithm to generate the semantic identifier.
    
    To generate the encoding, we leverage the base variant of a SentenceT5 model following DSI.
    We believe this superior to NCI where they use the simpler pretrained BERT-base.
    
    The hierarchical $k$-means setup follows that of NCI.
    More specifically, given the encodings, $k$-means is run to first generate $k$-clusters of documents.
    For clusters with at most $c$ documents, each document is assigned a number starting from $0$ to at most $c - 1$.
    For clusters with more than $c$ documents, the entire setup is run recursively, considering only those texts in the cluster.
    This terminates when there is a cluster satisfying the aforementioned condition of having at most $c$ documents.
    
    We consider an arbitrary document $d$, which when we run through this process, results in an assignment to the $9$th, $21$st, $14$th and $29$th cluster in sequential order.
    The resulting semantic identifier for such a document would be ``$[0,9]$ $[1,21]$ $[2,14]$ $[3,29]$'' and each of these $[i,j]$ identifiers indicate $j$-th cluster assignment in the $i$-th step (0-indexed).
    These identifiers are included in the vocabulary as an atomic unit.
    We dub identifiers leveraging this sort of additional ``index'' information as positional identifiers.
    Without positional identifiers, a $j$ at index $i_1$ is the same token as a $j$ at any other index $i_2$, making it harder for the decoder to capture.
    
    In our small scale experiments, we set the limits of $i$ and $j$ to be $4$ and $29$, respectively, while for our large scale experiments, we set them to be $8$ and $29$, respectively.
    This follows from the choice made by~\citet{Wang2022ANC} of $(k, c) = (30, 30)$.
    
    In the case that we use the entire MS MARCO Passage Ranking corpus, which totals to about 8.8M passages, we employ another strategy to make it computationally feasible.
    We first sample a million passages randomly and generate the semantic identifiers for those passages.
    This identifier serves as a sort of prefix identifier, for all the passages in the corpus and the same clustering process is running as was originally.
    Given that the initial set of seed clusters, will bifurcate the space of documents into smaller subsets, we can more easily run this process at scale.
    
    In this setting, to match the Neural Corpus Indexer setting, the output vocabulary only spans the different semantic identifiers introduced along with control tokens like the padding and end-of-sequence tokens.
    The token embeddings corresponding to the semantic identifiers are randomly initialized during model training. 
    
\end{itemize} 
\subsection{Document As Query (DAQ)}
To account for large Wikipedia articles in the Natural Questions and TriviaQA corpus, we leverage Document As Query, as seen in NCI~\cite{Wang2022ANC}.
More specifically, besides the standard DSI indexing task, where we consider only the first 64 tokens of each document, DAQ instead randomly selects 10 groups of 64 consecutive terms from the whole articles as additional queries.
This is akin to a form of randomized MaxP where we get better exposure of the document under consideration, given the first 64 tokens are often limiting to get a full picture of the entire Wikipedia article.
The result is a task besides the standard indexing task, which takes on the same input template albeit with segments from different parts of the article.
\subsection{Query Generation with doc2query--T5}
The generation and indexing tasks take on different data distributions -- queries are short, single-sentence long and request specific information while documents are multi-sentence long and convey information.
While the model is exposed to the entire corpus during the training phase through the indexing task, in most corpora, we do not have provided queries corresponding to the entire corpora.
For the MS MARCO passage ranking task, only 500K passages of the 8.8M in the corpus have a corresponding question in the training set.

To address this drift between the indexing and generation task, following~\cite{Wang2022ANC} we include another generation task which leverages generated queries from the doc2query--T5 model~\cite{nogueira2019docT5query}.
More specifically, first, for a particular document $d$ with identifier \emph{id}, the query generator, doc2query--T5, is used to generate queries that it finds relevant to the document.
These queries can serve as input to the DSI generation task, and the corresponding document identifier, $\emph{id}$, part of the target.

For the Natural Questions and TriviaQA datasets, we use the queries provided by~\citet{Wang2022ANC} to attempt to closely reproduce their results, totalling to about 20 and 15 queries per article, respectively.
It is worth noting that the query generation model used here was one trained on the MS MARCO passage ranking task and thus potentially faces some distributional effects coming from the shift from the relevance ranking source task and question answering target task.
Besides the standard query generator, we also leverage our model trained in the target task.


For the MS MARCO passage ranking subsets considered, we utilize the resource provided by~\citet{Ma2022DocumentEB}, where 40 queries for each passage in the corpora are included.
This used the same doc2query--T5 albeit where the training and evaluation datasets match.

\subsection{Prefix-Aware Weight-Adaptive Decoder (PAWA)}
From this subsection, we focus our attention on the semantic identifier setting, since that is the focus of~\citet{Wang2022ANC}.
The task of Neural Corpus Indexer with model parameters $\theta$ is to take an input query or document, both of which we represent with $q$, and generate the corresponding semantic identifier $s = s_1 \ldots s_m$
Hence, the probability of generating such an identifier can be denoted as:
\begin{equation}
    P(s\mid x,\theta) = \prod_{i=1}^m P(s_i \mid x, s_1, s_2, \ldots, s_{i-1}, \theta_i)
\end{equation}
\noindent where $x$ is the representation of $q$ from the encoder and $\theta_i$ is the model parameter at step $i$.
In the semantic setting for DSI, this was modeled with decoder based on T5.
More specifically:
\begin{equation}
    h_i = \text{T5Decoder}(x, h_1, \ldots, h_{i-1}; \theta_i)
    \label{eq:dec}
\end{equation}
\begin{equation}
    P(s_i \mid x, s_1, \ldots, s_{i-1}, \theta_i) = \text{softmax}(Wh_i)
    \label{eq:declin}
\end{equation}
\noindent where $h_i$ is the hidden representation for step $i$ and $W\in\mathbb{R}^{v \times d}$ is the final linear classifier mapping to the vocabulary space.

Following NCI, we disentangle the encoder and decoder vocabulary spaces instead of sharing since the model outputs identifiers instead of natural language.
In the decoder side, we ensure that the input vocabulary matrix and final linear classifier share weights.

The motivation of the PAWA decoder comes from an aspect in the semantic identifier generation stage that is not best accounted in the standard T5 decoder -- the Neural Corpus Indexer has to be flexible to capture different semantics with different prefixes.
For instance, take two sequences like ``$[0, 5]$ $[1, 14]$ $[2, 2]$'' and ``$[0, 6]$ $[1, 9]$ $[2, 2]$''.
The $[2, 2]$ while being the same token has different semantic meaning, given the prefixes are different.
Yet, the final linear classifier is static and fails to dynamically distinguish this identifier based on the prefix.

To solve this,~\citet{Wang2022ANC} propose enhancing the linear classification layer to be prefix-aware.
This is achieved with the addition of another transformer decoder:
\begin{equation}
    W_i^{pawa} = W \times \text{PawaDecoder}(s_1, \ldots, s_{i-1}) 
\end{equation}
where $W_i^{pawa} \in \mathbb{R}^{v \times d}$.
In our case, the PawaDecoder is another T5-based decoder of the same model size followed by a linear classifier. 
The resultant output is reshaped to form another linear classifier that can map the original weight matrix to the dynamic $W_i^{pawa}$.
Finally, we calculate the $i$-th token in the semantic identifier with $\text{softmax}(W_i^{pawa}h_i)$, where $h_i$ is the aforementioned hidden representation from the standard T5 decoder.
This choice is made based on open-sourced implementation by~\cite{Wang2022ANC}.
It is worth clarifying that this PAWA decoder is a Decoder-only model, given that it does not use the encoded representation from the encoder.
\subsection{Constrained Decoding}
In the standard inference stage, we use beam search to get the top-$k$ documents.
However, it is possible that the model generates a semantic identifier that does not correspond to any document in the corpus.
To account for this, the Neural Corpus indexer leverages constrained decoding where they constrain the beam search decoding process with a prefix tree corresponding to all document identifiers.

We account for the same by leveraging a Trie to hold all valid semantic identifiers and ensuring to go down beams that are valid.
We use a beam size of $100$ and a brevity penalty set to $0.0$ given that identifiers of different lengths are equally preferred.

\subsection{Consistency Loss - Regularization}
To help alleviate model over-fitting,~\citet{Wang2022ANC} propose employing a consistency-based regularization loss for each decoding step.
Two variants of this loss are suggested in different versions of the paper, both of which we consider.

For both variants, the input query $q$ is first run through the neural corpus indexer with two independent forward passes (with dropout affecting different parameters) prior to give two decoder representations prior to the final classification layer and softmax, at a particular step $i$, $h_{i,1}$ and $h_{i,2}$.
This is governed by Equation~\ref{eq:dec}.

Once this is calculated, the first loss considered tries to maximize the inner product between the same representations corresponding to the same input query $q$ while minimizing the inner product with all other queries considered in the batch ($B$), leveraging the softmax loss at each decoding step.
More specifically, the first regularization loss explored is defined as:
\begin{equation}
    \mathcal{L}_{reg, 1} = - \text{log} \frac{\text{exp}{(h_{i,1} \cdot h_{i,2})}}{\sum_{k=2}^{2|B|}\text{exp}(h_{i,1} \cdot h_{i,k})}
\end{equation}
where we are basically summing over the exponentiation of all inner products that can be computed with decoder representations from every other forward pass of different queries in the batch.
The $2|B|$ upper bound of the summation comes from the fact that each query in the batch has two independent forward passes.

Another variant proposed in another version of the paper, uses the Kullback-Leibler (KL) Divergence between the output probabilities of two independent forward passes, at each step.
More specifically, suppose $p_{i,1}$ and $p_{i,2}$ are the probability distributions over the vocabulary space after $h_{i,1}$ and $h_{i,2}$ are passed through Equation~\ref{eq:declin}).
Then, the bidirectional KL-based consistency loss at each step is given by:
\begin{equation}
    \mathcal{L}_{reg, 2} =  \tfrac{1}{2} \cdot [D_{KL}(p_{i,1} \mid \mid p_{i,2}) + D_{KL}(p_{i,2} \mid \mid p_{i,1})]
\end{equation}

Both of these loss functions are independently combined with the standard teacher-forcing cross entropy objective with weights $0.15$ and $0.015$ assigned to $\mathcal{L}_{reg, 1}$ and $\mathcal{L}_{reg, 2}$, respectively.
While we attempt to match our experimental setup as closely as we can with both variants in the Neural Corpus Indexer codebase, we find that training with this additional objective leads to training instability and the model effectiveness diverges into a NaN loss.
We explore other smaller weight choices and noted similar effectiveness drops and decide to not include consistency regularization in our final experimental setup.
% \subsection{Contrastive Learning - Losses}
% \subsection{Listwise In-Context DSI}





==> results.tex <==

\section{Results Old}\label{sec.results}
%\input{tab_nci_small_scale}


\subsection{Research Questions}\label{sec.questions}
In this section, we attempt to answer the following research questions through experiments. 


%\paragraph{R1. Can the results from NCI be replicated?}

\paragraph{R1. How effective is the generative retrieval model at different scales?}

\paragraph{R2. What is the most-effective model configuration?}

\paragraph{R3. How vital is question generation?}

\subsection{Generative Retrieval Model at Scales}\label{sec.questions}

The results on NQ100K and TriviaQA are summarised in Table~\ref{table:v1:nci_small_scale},
and the results for the MS Marco variants are in Table~\ref{table:v1:passage_subset}.
The first block includes the baseline results where results from the literature are directly used.
In the second block, we include results for both DSI and NCI at a small scale.  
In the third block of both tables, the results focus on the use of D2Q only as document representation,
and demonstrate its strength as document representation alone. 

%\paragraph{R1. Can the results from NCI be replicated?}
%
%\noindent The short answer is yes.
%Our replication results for NCI is in row (5).
%It can be seen that  
%we achieve slightly better results than the ones reported in NCI on NQ100K and performed on-par 
%on TriviaQA.
% On NQ100K, after adding D2Q (3a) as the document representation,
%the result is already above the reported results in NCI (b3). 
%Whereas, on TriviaQA, our results are three points 
% behind the NCI results. However, this is due to 
% the NCI results being from a corrupted input file and 
% being mistakenly reported on TriviaQA.
%
%


%  The mixture task indicated in row (2d) represents the task that is leveraged in the final NCI model, the effectiveness of which is reported in row (1c).


\paragraph{R1. How effective is the generative retrieval model at different scales?}

At large scale, the short answer is \emph{no}: Neither DSI nor NCI can outperform the dual-encoder baselines.

According to row (5) in Table~\ref{table:v1:passage_subset}, both DSI and NCI base variants underperform BM25 (b1) and dual encoder model GTR~\cite{ni22gtr} by a large margin.
 
On the one hand, it can be seen that the results look quite different when 
switching from Wikipedia-based NQ100k and TriviaQA (from Table~\ref{table:v1:nci_small_scale}) to MS Marco, even on smaller
variants.
DSI and NCI could provide a $4 \times$ effectiveness boost on NQ100K, and $30\%+$ improvement on TriviaQA.
When moving to MS Marco 100K and 1M, DSI can only perform ~30\% of BM25's results. 
While NCI could still outperform BM25, the margin shrinks considerably, from +50\% to ~20\%, and lacks behind the dual-encoder baseline by a margin.
On the other hand, 
when scaling up to the full dataset,
these two could barely provide half of the results of BM25, highlighting 
the difficulties in scaling up generative retrieval models on corpus at scales.



\paragraph{R2.  What is the best-performed model configuration?}

\noindent The short answer is Atomic or Naive DocIDs along with question generation
contribute to the best configuration.
To do that, we leverage observations at small-scale experiments,
coming up with a recipe by simply cherry-picking different configurations described
in Section~\ref{sec.methods}.
We add in individual components to see if they bring in improvements and we can stop wherever in the list of components if it leads to a drop in effectiveness. 
We show two findings about the model design empirically. 


\paragraph{F1. Atomic and Naive IDs are preferable.}

\noindent Atomic IDs are better if without considering the required larger model size,
and naive IDs are better if we use models of the same size.

On all datasets, it is clear that atomic DocID brings in 
the best performance, even after adding PAWA and constrained decoding
on top of the 2D Semantic IDs.
However, it is very important to consider that the atomic IDs
require extra model parameters to store all document identifiers in its vocabulary,
leading to an additional 7 billion model parameters compared to something like the naive sequential setting at most.
Among the naive IDs and (2D) semantic IDs, the naive identifier performs 
at least on par on all datasets, but without the extra computation required to generate the semantic IDs and the curated model changes like PAWA and constrained decoding.




\paragraph{F2. D2Q is essential for large-scale corpora.}

%As in the NCI paper, we focus on the semantic DocIDs setting.
It can be seen that the use of D2Q brings 10\% plus performance jump (3a vs 2b) on both datasets.
% Compared with FirstP, DaQ is more effective by a small margin (2b vs 2a), as a result of its use of the full
%document content instead of just the first 64 terms.
%In the meantime, constrained decoding does not help on TriviaQA, when contributing marginal 
%boosts on NQ100K (4b vs 4a).
It can be seen that, among different configurations, D2Q contributes the most, and DaQ is more effective than FirstP. As for the model building blocks from Section~\ref{sec.nci}, PAWA with 2D semantic DocID, constrained decoding do not contribute positively.
The best results were achieved after removing all of the components and only using D2Q and atomic IDs in the task mixture (6b). This is consistent among all three MS Marco variants.
On MSMarcoFULL, 
the best results outperform BM25 by 30\%. However, it is still well behind the GTR results (-30\%), and
11\% worse than BM25 with docT5query.


%scale up from 100k to full MS Marco corpus with 8.8M passages. On MSMarco100K and MSMarco1M, DSI (row (2a)) gets close to BM25 whereas NCI (row (5)) is well above BM25. The gap 
%%, though with smaller margin (~20\% better vs +50\% better in Table~\ref{table:v1:nci_small_scale}). 



% In this section, we attempt to answer the following research questions based on our experiments.
% To this mixture, we see that adding synthetic queries from doc2query--T5 (row (2c)) further improves effectiveness and in the NQ dataset we are already over the reported results of the full NCI model described in~\citet{Wang2022ANC} across the document identifier settings.
%     This demonstrates the vitality of synthetic query generation towards building a Neural Corpus Indexer, despite the fact that these Wikipedia articles have multiple questions in the training set for most of the passages in the corpus.

% \paragraph{R1. Can the effectiveness of Neural Corpus Indexer be replicated on the question answering datasets --- Natural Questions and TriviaQA?}

% \begin{itemize}
%     \item Note: Unlike NCI, we build our setup ground up from a T5-base sequence-to-sequence model and the Document as Query task.
%     We add in individual components to see if they bring in improvements and we can stop wherever in the list of components if it leads to a drop in effectiveness. 
%     It is also worth noting that we evaluate across the other document identifier settings considered by~\citet{Tay2022TransformerMA}, that is atomic and naive, given that these are not properly evaluated by~\citet{Wang2022ANC}.
%     We believe that these comparisons are required to determine which document identifiers work well and guide future work.
%     \item \emph{R1a. What is the importance of each task in the base NCI model?}\\
%     Rows (2a)--(2d) in Table~\ref{table:v1:nci_small_scale} form the base NCI model (that is a standard T5-base) with different tasks added one by one into the mixture task.
%     The mixture task indicated in row (2d) represents the task that is leveraged in the final NCI model, the effectiveness of which is reported in row (1c).
%     It is worth noting that the settings denoted in rows (2a)--(2d) \emph{do not} include the modeling components like PAWA, Constrained Decoding or Consistency Loss.
    
%     We begin with the zero-shot indexing ``Document As Query'' task (row (2a)), and then add the standard generation task with training query set (row (2b)).
%     As is seen this mixture demonstrates much higher effectiveness than zero-shot setting.
%     This demonstrates that it is crucial at the moment to also include some task that does not drift from the standard query form, to build a Neural Corpus Indexer.
    
%     To this mixture, we see that adding synthetic queries from doc2query--T5 (row (2c)) further improves effectiveness and in the NQ dataset we are already over the reported results of the full NCI model described in~\citet{Wang2022ANC} across the document identifier settings.
%     This demonstrates the vitality of synthetic query generation towards building a Neural Corpus Indexer, despite the fact that these Wikipedia articles have multiple questions in the training set for most of the passages in the corpus.
    
%     Additionally, we find that incorporating the indexing the first 64 tokens of the whole document in the mixture (row (2d)), while displaying slightly better effectiveness in most settings, does not seem significant and consistent.
%     While this is not significant, in these two datasets, to keep our setting comparable to that of~\citet{Wang2022ANC}, we choose to stick with this setting for modeling variants.
%     \item \emph{R1b. What role does PAWA play in our Neural Corpus Indexer Reproduction?}\\
%     Table~\ref{table:v1:nci_small_scale} row (3a) represents the effectiveness of the model when the PAWA decoder is added to the model and task mixture denoted in row (2d).
%     TODO(ronakpradeep) include few lines about how many more model parameters.
    
%     As can be seen, while this introduces a lot of model parameters, we seem to note a small drop in effectiveness.
%     It is worth noting however, that the when comparing the learning curves of both these rows, the curve of the model with the PAWA decoder is a lot ahead and converges quicker than the curve of that without.
%     This could however be attributed to the parameter increase, as similar benefits are seen when switching to the atomic setting.
%     Based on our results, it does not seem that such a variant of the Prefix-Aware Weight-Adaptive Decoder is vital to building a Neural Corpus Indexer for these datasets.
%     \item \emph{R1c. Is constrained decoding important for semantic identifiers?} \\
%     It seems very plausible that constrained decoding is vital for improved effectiveness in the semantic identifiers setting, given that most of the semantic identifier space, i.e., the $\approx 30^4$ (30 possible semantic identifier token outputs at each step and at most 4 steps) possible identifiers do not correspond to any passage in the corpora.
%     However, as seen in Table~\ref{table:v1:nci_small_scale}, this is not the case, and we only note a small bump in effectiveness.
%     This aligns with the results noted by~\citet{Wang2022ANC}, albeit they note a slightly bigger improvement.
%     This suggests that our model learns to properly decode sticking to valid identifiers in the semantic space, erring only occasionally.
 
%     \item \emph{R1d. Which document identifier works best?} \\
%     We find that Atomic DocIDs display the highest effectiveness across the three settings.
%     However, these identifiers come with an increase of about $768 \times |\mathcal{C}| \approx 80M$ model parameters in these datasets.
%     Hence, it is imperative to consider these results with the caveat that the increased parametric count might benefit the model.
%     Also, unlike the Neural Corpus Indexer paper it seems like adding semantic identifiers does not help improve the end effectiveness even compared to the naive sequential identifiers.
%     This brings to question a lot of what we are trying to achieve with semantic identifiers and it remains to be seen how to generate ``helpful'' semantic representations for these tasks. 
% \end{itemize}

% \paragraph{R2. Do these findings transfer to the MS MARCO Passage Relevance Ranking Task and at different scales?}
% \begin{itemize}
%   \item
%     Firstly,  it is worth noting that not all settings transfer to the MS MARCO passage ranking task.
%     The document as query setting only makes sense in a document ranking task, given that in the passage ranking tasks, passages are on average at most 128 tokens which fits the paradigm without multiple segments of the passage.
%     Hence, the base zero-shot setting is the standard indexing task with the passage as the retrieval unit.
%     \item R2a. Are similar trends noted in the MS-100K setting compared to the Question Answering datasets of comparable corpora sizes?\\
%     Rows (2a)--(2e) in Table~\ref{table:v1:passage_subset} explore the effectiveness of the base NCI model with various tasks and mixtures in the MS MARCO Passage Ranking task.
%     Limiting our observations to the columns of the MS-100K, in the atomic case, we see that exposing the model to just the indexing task, completely fails to capture the evaluation generation task in a zero-shot manner (row (2a)).
%     However, using either the naive or semantic sequential identifiers helps the model learn a weak representation for this task.
    
%     Adding the training query set generation task (row (2b)), we see a boost in effectiveness for the sequential identifier settings, however, the atomic setting still results in a model incapable of capturing the target task.
%     This diverges from the findings in the Natural Questions and TriviaQA datasets, where such a mixture, row (2b) in Table~\ref{table:v1:nci_small_scale} demonstrates effectiveness somewhat comparable to our best models, while here the model effectiveness is still sub-par.
    
%     Incorporating the generated query set into this mixture, seems to be the most crucial addition, as can be see in row (2c).
%     This boosts the learning of an effective neural corpus indexer across all cases, although especially in the atomic case where the model suddenly performs considerably better than the other sequential models.
    
%     Given the vitality of doc2query--T5 in this recipe for the MS MARCO passage ranking tasks, we consider two additional settings --- NCI\textsubscript{d2q}, where we only consider generation task with the synthetic query set and NCI\textsubscript{idx + d2q}, where we add the indexing task into the mixture (rows (2d) and (2e), respectively).
%     We can see from row (2d) that for the most part, it suffices to just train the model on the generation task with the synthetic query set. 
%     This is because the additions of other tasks, as seen in rows (2c) and (2e), do not seem critical to model effectiveness.
    
%     We look at results of the addition of PAWA to our most effective model, NCI\textsubscript{d2q}.
%     As can be seen in row (3a), the use of PAWA like the Natural Questions and TriviaQA case does not seem vital to better effectiveness of the final model.
%     Here too, however, we note that the addition results in much quicker convergence, given that the PAWA architecture also likely adds some model parameters making it more effective with fewer training steps.
    
%     Constrained decoding in this setting too brings about only a tiny boost in effectiveness, as can be seen comparing rows (2d) and (3b) for the MS-100K setting.
%     This demonstrates that the model already captures the notion of only decoding in the semantic identifier space without the constraints.
    
%     Our best model, NCI\textsubscript{d2q} with atomic identifiers, demonstrates effectiveness higher than BM25 (row (1a)) although only comparable to BM25 + doc2query--T5 (row (1b)).
%     Some more breakthroughs are required to Neural Corpus Indexers before the demonstrate effectiveness comparable to a model like GTR-base (row (1c)), although this represent a very powerful dual encoder and unified generative models are still in their infancy.
    
%     It is interesting to note that among identifiers, here too, we see that atomic identifiers outperform the sequential kinds.
%     Among the sequential identifiers, it seems like leveraging naive identifiers are slightly more effective than semantic identifiers. 
%     However, in the case of a task like MS MARCO passage ranking, these naive sequential identifiers often capture some notion of semantics as one can find multiple identifiers relevant to a query that are close in the identifier space.
%     \item R2b. How does scaling to MS-Full effect the findings?\\
%     Firstly, the general trends seem to continue as we scale towards the MS MARCO full setting.
%     It is worth noting that training these models takes considerably longer, 9M steps as opposed to 1M steps at most before convergence in the small scale experiments.
%     This makes sense given we are trying to index collections of $90 \times$ the passage count.
%     The training query set generation tasks in isolation do not seem to useful to the standard indexing task, given it only exposes generation of a small set of training queries, covering less than $10\%$ of the corpus.
    
%     With the addition of the PAWA decoder (row (3a)), the model converges a lot quicker than the case without (row (2d)).
%     This plays an even bigger role in the MS-full case given that the semantic model does not fully converge even after the $9M$ steps set out for the model, meanwhile the PAWA model hits an effectiveness of 14.0 before.
%     Hence, it seems like the PAWA architecture does help to some degree with scale, in training an effective neural corpus indexer faster.
%     However, this comes with the added model complexity and the PAWA model is still behind the naive string identifier solution without any such architectural modifications (row (2e)).
    
%     While it might seem like atomic identifiers significantly outperform the other two sequential identifiers with scale, it is very important to consider that this setting leads to a model of an additional 7 billion model parameters compared to something like the naive sequential setting.
%     Among the sequential identifiers, the naive identifier seems to lead to the most effective Neural Corpus Indexer, albeit with the aforementioned caveat that these ``naive'' identifiers capture some notion of semantics in the MS MARCO passage ranking task.
% \end{itemize}

%\input{tab_msmarco_subsets}
%\input{tab_msmarco_loss}
%\input{tab_msmarco_group}
%\input{tab_msmarco}


% \paragraph{R3. What does scaling behold?}
% \begin{itemize}
%     \item R3a: Table~\ref{table:v1:passage_full} explores this in the MS MARCO full setting, using 90 times the corpus size as the other corpora considered.
%     \item R3b: Scaling Laws: Base vs.\ XL
% \end{itemize}

% \paragraph{R4. The effect of better query generation}
% \begin{itemize}
%     \item R4a: Table~\ref{table:v1:passage_full} explores this in the MS MARCO full setting, using 90 times the corpus size as the other corpora considered.
%     \item R4b: Scaling Laws: Base vs.\ XL
% \end{itemize}

%% original
% \paragraph{R1. What is the effectiveness of Vanilla DSI and Neural Corpus Indexer on MS Marco?}
% \begin{itemize}
%     \item R1a. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs. (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c)).
%     \item R1b: Compare across MS100k, MS500k, MS1M, and MS-Full subsets (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c) and Table~\ref{table:v1:passage_full}, row (2a)).
%     \item R1c. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c), (3a) and Table~\ref{table:v1:passage_full}, row (2a), (3a)).
%     We scale only the best of the two IDs.
%     % \item R1c. Empirical findings, e.g., warning-up 
% \end{itemize}

% \paragraph{R2. What role does Query Generation play in Neural Corpus Indexer.}
% \begin{itemize}
%     \item R2a. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, rows (2d)--(2e) and Table~\ref{table:v1:passage_full}, row (2b)).
%     \item R2b. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3b) and Table~\ref{table:v1:passage_full}, row (3b)).
%     \item R2c. Overlap of the generated questions with the actual test questions.
%     % \item R2d. Replace query generation with text chunking. 
% \end{itemize}


% \paragraph{R3. Do sequential generalizations of L2R losses help?}
% \begin{itemize}
%     \item R3a. Choice of loss functions (Table~\ref{table:v1:passage_loss}).
%     \item R3b. Choice of hard negative group size and source (Table~\ref{table:v1:passage_group}, rows (1a)--(1e) and (2a)--(2e)).
%     Perhaps, we can simplify to only 2, 8, and 16 group size.
%     Need to see if source of hard negatives matter.
%     \item R3c. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, row (2f) and Table~\ref{table:v1:passage_full}, row (2c)).
%     \item R3d. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3c) and Table~\ref{table:v1:passage_full}, row (3c)).
% \end{itemize}

% \paragraph{R4. Can in-context negatives/hard-negatives increase effectiveness? (only in the Atomic DocIDs case, as atomic tokens)}
% \begin{itemize}
%     \item R4a. Choice of hard negative group size and source (Table~\ref{table:v1:passage_group}, rows (1f)--(1j) and (2f)--(2j)).
%     Perhaps, we can simplify to only 2, 8, and 16 group size.
%     Need to see if source of hard negatives matter.
%     \item R4b. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, row (2g) and Table~\ref{table:v1:passage_full}, row (2d)).
%     \item R4c. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3d) and Table~\ref{table:v1:passage_full}, row (3d)). 
% \end{itemize}
% \input{tab_nq}

==> results_backup.tex <==
\section{Results}\label{sec.results}
\input{tab_nci_small_scale}


In this section, we attempt to answer the following research questions based on our experiments.

\paragraph{R1. Can the effectiveness of Neural Corpus Indexer be replicated on the question answering datasets --- Natural Questions and TriviaQA?}

\begin{itemize}
    \item Note: Unlike NCI, we build our setup ground up from a T5-base sequence-to-sequence model and the Document as Query task.
    We add in individual components to see if they bring in improvements and we can stop wherever in the list of components if it leads to a drop in effectiveness. 
    It is also worth noting that we evaluate across the other document identifier settings considered by~\citet{Tay2022TransformerMA}, that is atomic and naive, given that these are not properly evaluated by~\citet{Wang2022ANC}.
    We believe that these comparisons are required to determine which document identifiers work well and guide future work.
    \item \emph{R1a. What is the importance of each task in the base NCI model?}\\
    Rows (2a)--(2d) in Table~\ref{table:v1:nci_small_scale} form the base NCI model (that is a standard T5-base) with different tasks added one by one into the mixture task.
    The mixture task indicated in row (2d) represents the task that is leveraged in the final NCI model, the effectiveness of which is reported in row (1c).
    It is worth noting that the settings denoted in rows (2a)--(2d) \emph{do not} include the modeling components like PAWA, Constrained Decoding or Consistency Loss.
    
    We begin with the zero-shot indexing ``Document As Query'' task (row (2a)), and then add the standard generation task with training query set (row (2b)).
    As is seen this mixture demonstrates much higher effectiveness than zero-shot setting.
    This demonstrates that it is crucial at the moment to also include some task that does not drift from the standard query form, to build a Neural Corpus Indexer.
    
    To this mixture, we see that adding synthetic queries from doc2query--T5 (row (2c)) further improves effectiveness and in the NQ dataset we are already over the reported results of the full NCI model described in~\citet{Wang2022ANC} across the document identifier settings.
    This demonstrates the vitality of synthetic query generation towards building a Neural Corpus Indexer, despite the fact that these Wikipedia articles have multiple questions in the training set for most of the passages in the corpus.
    
    Additionally, we find that incorporating the indexing the first 64 tokens of the whole document in the mixture (row (2d)), while displaying slightly better effectiveness in most settings, does not seem significant and consistent.
    While this is not significant, in these two datasets, to keep our setting comparable to that of~\citet{Wang2022ANC}, we choose to stick with this setting for modeling variants.
    \item \emph{R1b. What role does PAWA play in our Neural Corpus Indexer Reproduction?}\\
    Table~\ref{table:v1:nci_small_scale} row (3a) represents the effectiveness of the model when the PAWA decoder is added to the model and task mixture denoted in row (2d).
    TODO(ronakpradeep) include few lines about how many more model parameters.
    
    As can be seen, while this introduces a lot of model parameters, we seem to note a small drop in effectiveness.
    It is worth noting however, that the when comparing the learning curves of both these rows, the curve of the model with the PAWA decoder is a lot ahead and converges quicker than the curve of that without.
    This could however be attributed to the parameter increase, as similar benefits are seen when switching to the atomic setting.
    Based on our results, it does not seem that such a variant of the Prefix-Aware Weight-Adaptive Decoder is vital to building a Neural Corpus Indexer for these datasets.
    \item \emph{R1c. Is constrained decoding important for semantic identifiers?} \\
    It seems very plausible that constrained decoding is vital for improved effectiveness in the semantic identifiers setting, given that most of the semantic identifier space, i.e., the $\approx 30^4$ (30 possible semantic identifier token outputs at each step and at most 4 steps) possible identifiers do not correspond to any passage in the corpora.
    However, as seen in Table~\ref{table:v1:nci_small_scale}, this is not the case, and we only note a small bump in effectiveness.
    This aligns with the results noted by~\citet{Wang2022ANC}, albeit they note a slightly bigger improvement.
    This suggests that our model learns to properly decode sticking to valid identifiers in the semantic space, erring only occasionally.
 
    \item \emph{R1d. Which document identifier works best?} \\
    We find that Atomic DocIDs display the highest effectiveness across the three settings.
    However, these identifiers come with an increase of about $768 \times |\mathcal{C}| \approx 80M$ model parameters in these datasets.
    Hence, it is imperative to consider these results with the caveat that the increased parametric count might benefit the model.
    Also, unlike the Neural Corpus Indexer paper it seems like adding semantic identifiers does not help improve the end effectiveness even compared to the naive sequential identifiers.
    This brings to question a lot of what we are trying to achieve with semantic identifiers and it remains to be seen how to generate ``helpful'' semantic representations for these tasks. 
\end{itemize}

\paragraph{R2. Do these findings transfer to the MS MARCO Passage Relevance Ranking Task and at different scales?}
\begin{itemize}
   \item
    Firstly,  it is worth noting that not all settings transfer to the MS MARCO passage ranking task.
    The document as query setting only makes sense in a document ranking task, given that in the passage ranking tasks, passages are on average at most 128 tokens which fits the paradigm without multiple segments of the passage.
    Hence, the base zero-shot setting is the standard indexing task with the passage as the retrieval unit.
    \item R2a. Are similar trends noted in the MS-100K setting compared to the Question Answering datasets of comparable corpora sizes?\\
    Rows (2a)--(2e) in Table~\ref{table:v1:passage_subset} explore the effectiveness of the base NCI model with various tasks and mixtures in the MS MARCO Passage Ranking task.
    Limiting our observations to the columns of the MS-100K, in the atomic case, we see that exposing the model to just the indexing task, completely fails to capture the evaluation generation task in a zero-shot manner (row (2a)).
    However, using either the naive or semantic sequential identifiers helps the model learn a weak representation for this task.
    
    Adding the training query set generation task (row (2b)), we see a boost in effectiveness for the sequential identifier settings, however, the atomic setting still results in a model incapable of capturing the target task.
    This diverges from the findings in the Natural Questions and TriviaQA datasets, where such a mixture, row (2b) in Table~\ref{table:v1:nci_small_scale} demonstrates effectiveness somewhat comparable to our best models, while here the model effectiveness is still sub-par.
    
    Incorporating the generated query set into this mixture, seems to be the most crucial addition, as can be see in row (2c).
    This boosts the learning of an effective neural corpus indexer across all cases, although especially in the atomic case where the model suddenly performs considerably better than the other sequential models.
    
    Given the vitality of doc2query--T5 in this recipe for the MS MARCO passage ranking tasks, we consider two additional settings --- NCI\textsubscript{d2q}, where we only consider generation task with the synthetic query set and NCI\textsubscript{idx + d2q}, where we add the indexing task into the mixture (rows (2d) and (2e), respectively).
    We can see from row (2d) that for the most part, it suffices to just train the model on the generation task with the synthetic query set. 
    This is because the additions of other tasks, as seen in rows (2c) and (2e), do not seem critical to model effectiveness.
    
    We look at results of the addition of PAWA to our most effective model, NCI\textsubscript{d2q}.
    As can be seen in row (3a), the use of PAWA like the Natural Questions and TriviaQA case does not seem vital to better effectiveness of the final model.
    Here too, however, we note that the addition results in much quicker convergence, given that the PAWA architecture also likely adds some model parameters making it more effective with fewer training steps.
    
    Constrained decoding in this setting too brings about only a tiny boost in effectiveness, as can be seen comparing rows (2d) and (3b) for the MS-100K setting.
    This demonstrates that the model already captures the notion of only decoding in the semantic identifier space without the constraints.
    
    Our best model, NCI\textsubscript{d2q} with atomic identifiers, demonstrates effectiveness higher than BM25 (row (1a)) although only comparable to BM25 + doc2query--T5 (row (1b)).
    Some more breakthroughs are required to Neural Corpus Indexers before the demonstrate effectiveness comparable to a model like GTR-base (row (1c)), although this represent a very powerful dual encoder and unified generative models are still in their infancy.
    
    It is interesting to note that among identifiers, here too, we see that atomic identifiers outperform the sequential kinds.
    Among the sequential identifiers, it seems like leveraging naive identifiers are slightly more effective than semantic identifiers. 
    However, in the case of a task like MS MARCO passage ranking, these naive sequential identifiers often capture some notion of semantics as one can find multiple identifiers relevant to a query that are close in the identifier space.
    \item R2b. How does scaling to MS-Full effect the findings?\\
    Firstly, the general trends seem to continue as we scale towards the MS MARCO full setting.
    It is worth noting that training these models takes considerably longer, 9M steps as opposed to 1M steps at most before convergence in the small scale experiments.
    This makes sense given we are trying to index collections of $90 \times$ the passage count.
    The training query set generation tasks in isolation do not seem to useful to the standard indexing task, given it only exposes generation of a small set of training queries, covering less than $10\%$ of the corpus.
    
    With the addition of the PAWA decoder (row (3a)), the model converges a lot quicker than the case without (row (2d)).
    This plays an even bigger role in the MS-full case given that the semantic model does not fully converge even after the $9M$ steps set out for the model, meanwhile the PAWA model hits an effectiveness of 14.0 before.
    Hence, it seems like the PAWA architecture does help to some degree with scale, in training an effective neural corpus indexer faster.
    However, this comes with the added model complexity and the PAWA model is still behind the naive string identifier solution without any such architectural modifications (row (2e)).
    
    While it might seem like atomic identifiers significantly outperform the other two sequential identifiers with scale, it is very important to consider that this setting leads to a model of an additional 7 billion model parameters compared to something like the naive sequential setting.
    Among the sequential identifiers, the naive identifier seems to lead to the most effective Neural Corpus Indexer, albeit with the aforementioned caveat that these ``naive'' identifiers capture some notion of semantics in the MS MARCO passage ranking task.
\end{itemize}

\input{tab_msmarco_subsets}
\input{tab_msmarco_loss}
\input{tab_msmarco_group}
\input{tab_msmarco}


% \paragraph{R3. What does scaling behold?}
% \begin{itemize}
%     \item R3a: Table~\ref{table:v1:passage_full} explores this in the MS MARCO full setting, using 90 times the corpus size as the other corpora considered.
%     \item R3b: Scaling Laws: Base vs.\ XL
% \end{itemize}

% \paragraph{R4. The effect of better query generation}
% \begin{itemize}
%     \item R4a: Table~\ref{table:v1:passage_full} explores this in the MS MARCO full setting, using 90 times the corpus size as the other corpora considered.
%     \item R4b: Scaling Laws: Base vs.\ XL
% \end{itemize}

%% original
% \paragraph{R1. What is the effectiveness of Vanilla DSI and Neural Corpus Indexer on MS Marco?}
% \begin{itemize}
%     \item R1a. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs. (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c)).
%     \item R1b: Compare across MS100k, MS500k, MS1M, and MS-Full subsets (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c) and Table~\ref{table:v1:passage_full}, row (2a)).
%     \item R1c. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, rows (2a)--(2c), (3a) and Table~\ref{table:v1:passage_full}, row (2a), (3a)).
%     We scale only the best of the two IDs.
%     % \item R1c. Empirical findings, e.g., warning-up 
% \end{itemize}

% \paragraph{R2. What role does Query Generation play in Neural Corpus Indexer.}
% \begin{itemize}
%     \item R2a. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, rows (2d)--(2e) and Table~\ref{table:v1:passage_full}, row (2b)).
%     \item R2b. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3b) and Table~\ref{table:v1:passage_full}, row (3b)).
%     \item R2c. Overlap of the generated questions with the actual test questions.
%     % \item R2d. Replace query generation with text chunking. 
% \end{itemize}


% \paragraph{R3. Do sequential generalizations of L2R losses help?}
% \begin{itemize}
%     \item R3a. Choice of loss functions (Table~\ref{table:v1:passage_loss}).
%     \item R3b. Choice of hard negative group size and source (Table~\ref{table:v1:passage_group}, rows (1a)--(1e) and (2a)--(2e)).
%     Perhaps, we can simplify to only 2, 8, and 16 group size.
%     Need to see if source of hard negatives matter.
%     \item R3c. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, row (2f) and Table~\ref{table:v1:passage_full}, row (2c)).
%     \item R3d. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3c) and Table~\ref{table:v1:passage_full}, row (3c)).
% \end{itemize}

% \paragraph{R4. Can in-context negatives/hard-negatives increase effectiveness? (only in the Atomic DocIDs case, as atomic tokens)}
% \begin{itemize}
%     \item R4a. Choice of hard negative group size and source (Table~\ref{table:v1:passage_group}, rows (1f)--(1j) and (2f)--(2j)).
%     Perhaps, we can simplify to only 2, 8, and 16 group size.
%     Need to see if source of hard negatives matter.
%     \item R4b. With Naive Sequential DocIDs, Semantic Sequential DocIDs, and Atomic DocIDs (Table~\ref{table:v1:passage_subset}, row (2g) and Table~\ref{table:v1:passage_full}, row (2d)).
%     \item R4c. Scaling Laws: Base vs.\ XL (Table~\ref{table:v1:passage_subset}, row (3d) and Table~\ref{table:v1:passage_full}, row (3d)). 
% \end{itemize}
% \input{tab_nq}

==> tab_d2q_count.tex <==
% https://tensorboard.corp.google.com/compare/ND40_K20_TEM100_4words:7398344249163767709,ND40_K10_TEM70_4words:2926266844311145496,ND40_K10_TEM100_4words:7935123903438797931,ND100_K10_TEM100_4words:4697201122617285572,ND40_K20_TEM100_0words:8987831870954689067,ND40_K10_TEM70_0words:49197640940670671,ND40_K10_TEM100_0words:3279964719075669856,ND100_K10_TEM100_0words:527378741412604288/?darkMode=true&forceSVG=true#timeseries
\input{tab_d2q_rankt5}
\begin{table}[t]
\centering\scalebox{0.95}{
\begin{tabular}{lccccc}
\toprule
& |Q| & RankT5 Filter   & Temp. & top-$k$ & MRR@10 \ \\
\toprule
(2a) & 100 & \checkmark & 1.0 & 10 & 82.1 \\
(1a) & 40 & $\times$ & 1.0 & 10 & 80.3 \\
(1b) & 100 & $\times$ & 1.0 & 10 & 82.4 \\
\midrule
(2a) & 40 & \checkmark & 1.0 & 10 & 79.6 \\
(2b) & 40 & $\times$ & 1.0 & 10 & 80.3 \\
(3a) & 40 & \checkmark & 0.7 & 10 & 76.7 \\
(3b) & 40 & $\times$ & 0.7 & 10 & 78.0\\
\midrule
(4a) & 40 & \checkmark & 1.0 & 20 & 80.0 \\
(4b) & 40 & $\times$ & 1.0 & 20 & 80.6 \\
\bottomrule
\end{tabular}
}
\vspace{0.25cm}
\caption{Using RankT5 filter and larger beam size on MS Marco dev set.}
\label{table:v1:passage_n_queries}
\end{table}



% origin version:
% \input{tab_d2q_rankt5}
% \begin{table}[t]
% \centering\scalebox{0.95}{
% \begin{tabular}{lccccc}
% \toprule
% & |Q| & RankT5 Filter   & Temp. & top-$k$ & MRR@10 \ \\
% \toprule
% (2a) & 100 & \checkmark & 1.0 & 10 & 82.1 \\
% (1a) & 40 & $\times$ & 1.0 & 10 & 79.6 \\
% (1b) & 100 & $\times$ & 1.0 & 10 & 82.4 \\
% \midrule
% (2a) & 40 & \checkmark & 1.0 & 10 & 79.6 \\
% (2b) & 40 & $\times$ & 1.0 & 10 & 80.3 \\
% (3a) & 40 & \checkmark & 0.7 & 10 & 76.7 \\
% (3b) & 40 & $\times$ & 0.7 & 10 & 78.0\\
% \midrule
% (4a) & 40 & \checkmark & 1.0 & 20 & 80.0 \\
% (4b) & 40 & $\times$ & 1.0 & 20 & 80.6 \\
% \bottomrule
% \end{tabular}
% }
% \vspace{0.25cm}
% \caption{Using RankT5 filter and larger beam size on MS Marco dev set.}
% \label{table:v1:passage_n_queries}
% \end{table}

==> tab_d2q_rankt5.tex <==
% https://tensorboard.corp.google.com/compare/setting1_filtered80:7161911783587222611,setting3_filtered60:1589838512167525202,setting3_filtered20:2429792177280585121,setting1_filtered60:1981592941799975297,setting1_filtered20:1762782531759835941,setting3_filtered80:3961509493686230777,setting3_filtered40:3061585010244115802,setting1_filtered40:3984393488025311875/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true&forceSVG=true&runFilter=setting1#timeseries

\begin{table*}[t]
\centering\scalebox{0.95}{
\begin{tabular}{lccc}
\toprule
& $\%$ Remain & Global  &  MRR@10 \ \\
\toprule
(1a) & 100 & - & 80.3 \\
\midrule
(2a) & 20 & \checkmark & 57.0  \\
(2b) & 40 & \checkmark & 66.4\  \\
(2c) & 60 &  \checkmark & 74.4 \\
(2d) & 80 & \checkmark &  78.7 \\
\midrule
(3a) & 20 & $\times$ & 68.0 \\
(3b) & 40 & $\times$  &  74.4  \\
(3c) & 60 & $\times$ & 77.0 \\
(3d) & 80 & $\times$ & 78.9 \\
\bottomrule
\end{tabular}
}
\vspace{0.25cm}
\caption{Results of ablating various aspects of RankT5 filtering for NCI\textsubscript{d2q} on the development set of MS-100K (Perhaps some stats in the side too).}
\label{table:v1:passage_rankt5}
\end{table*}

==> tab_method.tex <==
\begin{table}[]
    \centering\scalebox{0.9}{
    \begin{tabular}{c|c|c|c}
    \toprule
    & DSI & NCI & UGR \\
    \midrule
  \multicolumn{4}{c}{\textbf{Backbone: ranking as seq2seq tasks}} \\
    \midrule
         Indexing/generation tasks &\checkmark&\checkmark&\checkmark\\
         \midrule
         \multicolumn{4}{c}{\textbf{DocID variants}} \\
         \midrule
         Atomic DocID&\checkmark&& \\
         Naive DocID&\checkmark&&\checkmark  \\
         Semantic DocID&\checkmark&& \\
         2D Semantic DocID &&\checkmark& \\
         \midrule
           \multicolumn{4}{c}{\textbf{Document Representations}} \\
         \midrule
         First $k$ terms (FirstP) &\checkmark&\checkmark&\\
         Document-As-Query (DaQ) &&\checkmark&  \\
         QGen &&\checkmark&\checkmark  \\
          \midrule
          \multicolumn{4}{c}{\textbf{Model components from NCI}} \\
          \midrule
         PAWA &&\checkmark&  \\
         Consistency Loss &&\checkmark&\\
         Constrained Decoding &&\checkmark& \\
\bottomrule
    \end{tabular}}
    \vspace{0.25cm}
\caption{Overview of the components behind the methods considered.}
    \label{tab.method}
\end{table}

==> tab_msmarco.tex <==
% % Results for rows 2-4, a-c are in this tensorboard.
% % https://tensorboard.corp.google.com/compare/origin_dual_d2q_idx_full_t5base_naive_van_inplen128_wu100000:8479731151032329586,origin_d2q_full_t5base_naive_van_inplen128_wu100000:3169748956685540421,semantic_dual_d2q_idx_full_t5base_naive_van_inplen128_wu100000:193359840812812247,semantic_d2q_full_t5base_naive_van_inplen128_wu100000:4500277505996508356,semantic_d2q_full_t5base_naive_van_inplen128:956278554808777158,semantic_dual_d2q_idx_full_t5base_naive_van_inplen128:6333461814335071830,semantic_dual_rr32:8118433295503874007,semantic_index:8639710081609380594,origin_dual_d2q_idx_full_t5base_naive_van_inplen128:4351252062395499351,origin_d2q_full_t5base_naive_van_inplen128:2627469118534673643,origin_dual_rr32:3080278331267260145,origin_index:4670893756062752180,dual_rr32:7162752563992622430,dual_d2q:3970063584577856707,d2q:3908706769454919912/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true&smoothing=0#timeseries
% % Note that the models are yet to converge
% \begin{table*}[t]
% \centering\scalebox{0.8}{
% \begin{tabular}{lllccccc}
% \toprule
% & & & \multicolumn{2}{c}{\textbf{TREC 2019 DL Track}} & \multicolumn{2}{c}{\textbf{TREC 2020 DL Track}} & \multicolumn{1}{c}{\textbf{Dev}}\\
% \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
% & \multicolumn{2}{l}{{\bf Condition}} & AP & nDCG@10 & AP & nDCG@10 & RR@10 \\
% \toprule
% (1a) & \multicolumn{2}{l}{BM25} & 30.1 & 50.6 & 28.6 & 48.0 & 18.4\\
% (1b) & \multicolumn{2}{l}{BM25 (w/ doc2query--T5)} & 40.3 & 64.2 & 40.7 & 61.9 &  27.2 \\
% \midrule
% \multicolumn{3}{l}{\emph{Naive DocIDs}}\\ 
% (2a) & \multicolumn{2}{l}{DSI\textsubscript{idx}}  & & & & & 10.8 \\
% (2b) & \multicolumn{2}{l}{DSI\textsubscript{mix}} & & & & & 7.5 \\
% (2c) & \multicolumn{2}{l}{DSI\textsubscript{d2q}} & & & & & 11.8 \\
% (2d) & \multicolumn{2}{l}{LOSS-DSI\textsubscript{d2q}}  & & & & & 13.2 \\
% (2e) & \multicolumn{2}{l}{PROMPT-DSI\textsubscript{d2q}} \\
% \midrule
% \multicolumn{3}{l}{\emph{Semantic DocIDs}}\\ 
% (3a) & \multicolumn{2}{l}{DSI\textsubscript{idx}} & & & & & 1.1 \\
% (3b) & \multicolumn{2}{l}{DSI\textsubscript{mix}} & & & & & 2.1\\
% (3c) & \multicolumn{2}{l}{DSI\textsubscript{d2q}} & & & & & 8.0 \\
% (3d) & \multicolumn{2}{l}{DSI\textsubscript{d2q+idx}} & & & & & 1.8 \\
% (3e) & \multicolumn{2}{l}{LOSS-DSI\textsubscript{d2q}} \\
% (3f) & \multicolumn{2}{l}{PROMPT-DSI\textsubscript{d2q}} \\
% \midrule
% \multicolumn{3}{l}{\emph{Atomic DocIDs}}\\ 
% (4a) & \multicolumn{2}{l}{DSI\textsubscript{idx}} & & & & & 0.0  \\
% (4b) & \multicolumn{2}{l}{DSI\textsubscript{mix}} & & & & & 0.0 \\
% (4c) & \multicolumn{2}{l}{DSI\textsubscript{d2q}} & & & & & 19.4 \\
% (4d) & \multicolumn{2}{l}{DSI\textsubscript{d2q+idx}} & & & & & 1.8 \\
% (4e) & \multicolumn{2}{l}{LOSS-DSI\textsubscript{d2q}} \\
% (4f) & \multicolumn{2}{l}{PROMPT-DSI\textsubscript{d2q}} \\
% % \bottomrule
% % \multicolumn{3}{l}{\emph{T5-XL Variants}}\\ 
% % (3a) & \multicolumn{2}{l}{DSI\textsubscript{mix}} \\
% % (3b) & \multicolumn{2}{l}{DSI\textsubscript{d2q}} \\
% % (3c) & \multicolumn{2}{l}{LOSS-DSI\textsubscript{d2q}} \\
% % (3d) & \multicolumn{2}{l}{PROMPT-DSI\textsubscript{d2q}} \\
% \bottomrule
% \end{tabular}
% }
% \vspace{0.25cm}
% \caption{Results on the MS MARCO V1 passage corpus. }
% \label{table:v1:passage_full}
% \end{table*}

==> tab_msmarco_group.tex <==
% % Listwise prompt 
% % https://tensorboard.corp.google.com/compare/d2q_all_list32:5366389952794370286,dual_d2q_list32:3891901123843993280,d2q_all_list16:1423074477515294911,d2q_all_list8:3646832849546315787,dual_d2q_list16:8879182588664427591,dual_d2q_list8:6521900883721971768,dual_d2q_list4:3425256969546427620,d2q_all_list4:235503226978780465,d2q_all_list2:2827664008075400138,dual_d2q_list2:2312302106542239062/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true&runFilter=gen_nor#timeseries
% % We only use the single case where we use just the listwise task from scratch. Seems like cotraining didn't help here but varying results in some other settings I have explored. Will run first standard -> cotraining


% \begin{table*}[t]
% \centering\scalebox{0.8}{
% \begin{tabular}{llllrrr}
% \toprule
% & \multicolumn{3}{l}{{\bf Condition}} & At.\ & Nv.\ & Sm.\ \\
% \toprule
% \midrule
% \multicolumn{4}{l}{\emph{T5-base Variants}}\\
% (1a) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{2}} & 80.8 & 75.4  & 75.9 \\
% (1b) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{4}} & 80.9 & 74.4  & 75.3 \\
% (1c) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{8}} & 80.9 & 73.6 & 74.8 \\
% (1d) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{16}} & 80.9 & 72.7  & 74.3\\
% (1e) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{32}} & 80.8 & 72.2 & 73.7 \\
% (1f) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{2}} & 79.2 & -   & - \\
% (1g) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{4}} & 79.6 & -  & -\\
% (1h) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{8}} & 79.6  & -  & -\\
% (1i) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{16}} & 78.9 & -  & -\\
% (1j) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{32}} & 76.3 & -  & -\\
% % \midrule
% % \multicolumn{4}{l}{\emph{T5-XL Variants}}\\
% % (2a) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{2}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2b) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{4}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2c) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{8}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2d) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{16}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$\\
% % (2e) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{32}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2f) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{2}} & $w_{T1,3b}$ & -   & -  \\
% % (2g) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{4}} & $w_{T1,3b}$ & -  & - \\
% % (2h) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{8}} & $w_{T1,3b}$ & -  & - \\
% % (2i) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{16}} & $w_{T1,3b}$ & -  & - \\
% % (2j) & \multicolumn{3}{l}{PROMPT-CDSI\textsubscript{32}} & $w_{T1,3b}$ & -  & - \\
% \bottomrule
% \end{tabular}
% }
% \vspace{0.25cm}
% \caption{Results varying the group size on the 100K subset of the MS MARCO V1 passage collection (perhaps more fitting to eventually copy as a figure).}
% \label{table:v1:passage_group}
% \end{table*}

==> tab_msmarco_loss.tex <==
% % Results for this table

% % https://tensorboard.corp.google.com/compare/msid_d2q_train_only_group8_tiny_t5base_atomic_van_inplen128_contloss_d0:1697651719391768249,msid_d2q_train_only_group8_tiny_t5base_atomic_van_inplen128_contloss_ce_ul:7186891654882130905,msid_d2q_train_only_group8_tiny_t5base_atomic_van_inplen128_contloss_ce_ln:4110694191699909109,msid_d2q_train_only_group8_tiny_t5base_atomic_van_inplen128_contloss_lnonly:6635029889493587756,origin_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_d0:4698550167187720828,origin_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_ce_ul:5878596845369350687,origin_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_lnonly:6860189696224701002,origin_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_ce_ln:8732004113118531120,semantic_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_d0:5356185453437507736,semantic_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_ce_ul:758875640931574775,semantic_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_ce_ln:5957828051411344244,semantic_d2q_train_only_group8_tiny_t5base_naive_van_inplen128_contloss_lnonly:746935203160572609/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true#timeseries

% % need to properly examine losses again to scale up, getting negative loss is concerning.
% \begin{table*}[t]
% \centering\scalebox{0.8}{
% \begin{tabular}{llllrrr}
% \toprule
% & \multicolumn{3}{l}{{\bf Condition}} & At.\ & Nv.\ & Sm.\ \\
% \toprule
% \midrule
% \multicolumn{4}{l}{\emph{T5-base Variants}}\\
% (1a) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE}} & 80.3 & 78.7 & 78.5 \\
% (1b) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + UL}} & 80.8 & 75.1 & 75.8 \\
% (1c) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + LN}} & 80.9 & 78.6 & 78.5 \\
% (1d) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + UL + LN}} & 80.9 & 73.6 & 74.8 \\
% % \midrule
% % \multicolumn{4}{l}{\emph{T5-XL Variants}}\\
% % (2a) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2b) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + UL}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2c) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + LN}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% % (2d) & \multicolumn{3}{l}{LOSS-CDSI\textsubscript{CE + UL + LN}} & $w_{T1,3b}$ & $w_{T1,3b}$  & $w_{T1,3b}$ \\
% \bottomrule
% \end{tabular}
% }
% \vspace{0.25cm}
% \caption{Results varying the loss functions on the 100K subset of the MS MARCO V1 passage collection.}
% \label{table:v1:passage_loss}
% \end{table*}

==> tab_msmarco_xl.tex <==
% Base
% Tiny - Stage 1 - https://tensorboard.corp.google.com/compare/msid_dual_d2q:4858004084345797470,origin_dual_d2q:2907804120540135003,origin_d2q:3608780372607413139,semantic_dual_d2q:5477700722998981841,semantic_d2q:466325048530000343,msid_dual_tiny:5839897524485947917,msid_gen:4322247377687514615,msid_index:1770791123047805620,origin_dual_tiny:8395507286811246594,origin_gen:4966074175880556232,origin_index:9219005819868736691,semantic_dual_tiny:2475094185748348484,semantic_gen:1623985763033055856,semantic_index:8296920431808958911,msid_d2q:3356173368080982004/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true&runFilter=gen#timeseries

% Small - Stage 1 - https://tensorboard.corp.google.com/compare/msid_dual_d2q:8116336403829697820,msid_d2q:1772368193816378895,origin_dual_d2q:7177129894118710935,origin_d2q:1522705768227862753,semantic_dual_d2q:4334655565702269387,semantic_d2q:8537774637349266129,msid_dual_small:8994862242237467895,msid_gen:4622627048306858233,msid_index:5634067600575210001,origin_dual_small:387675313106761002,origin_gen:3795166331022819151,origin_index:7683215156164463844,semantic_gen:3501082783871112806,semantic_dual_small:8193298666715854988,semantic_index:7075902031519456085/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true&runFilter=semantic_#timeseries
% Medium (semantic generation ongoing) - Stage 1 - https://tensorboard.corp.google.com/compare/origin_d2q:3248219037680606571,origin_dual_d2q:4540434915169068185,d2q:3755776241339801421,dual_d2q:667691640987700576,dual_medium:1581948180985453809,gen:6502608519313541423,index:8757336141431383980,origin_dual_medium:2990693034843428277,origin_gen:1590395760749848168,origin_index:3947347393437038811/?pinnedCards=%5B%7B%22plugin%22%3A%22scalars%22%2C%22tag%22%3A%22eval%2Fmrr_10%22%7D%5D&darkMode=true#timeseries
\begin{table*}[t]
\centering\scalebox{0.8}{
\begin{tabular}{lllrrr}
\toprule
& & & \multicolumn{3}{c}{\textbf{MS-1M}}\\
\cmidrule(lr){4-6} 
& \multicolumn{2}{l}{{\bf Condition}} & At.\ & Nv.\ & Sm.\  \\
\toprule
\multicolumn{3}{l}{\emph{Baselines}}\\
(1a) & \multicolumn{2}{l}{BM25} & - & 65.3 &  - & - & 48.4 &  - & - & 41.3  & - \\
(1b) & \multicolumn{2}{l}{BM25 (w/ doc2query--T5)} & - & 80.4 &  - & - & 64.5 &  - & - & 56.6  & -\\
(1c) & \multicolumn{2}{l}{GTR-base} & - & 83.2 & - & - & 66.4 & - & - & 60.7 & - \\
(1d) & \multicolumn{2}{l}{GTR-XL} & - & 85.0 & - & - & 68.9 & - & - & 63.4 & -\\
\midrule
\multicolumn{3}{l}{\emph{T5-XL Variants}}\\
(3a) & \multicolumn{2}{l}{DSI\textsubscript{mix}} & $w_{2b}$ & $w_{2b}$  & $w_{2b}$  & $w_{2b}$  & $w_{2b}$ & $w_{2b}$  & $w_{2b}$  & $w_{2b}$ & $w_{2b}$ \\
(3b) & \multicolumn{2}{l}{DSI\textsubscript{d2q}} &  &   &   &  &   &   &   &  &   \\
(3c) & \multicolumn{2}{l}{LOSS-CDSI\textsubscript{d2q}}  & $w_{3b}$ & $w_{3b}$  & $w_{3b}$  & $w_{3b}$ &  $w_{3b}$ & $w_{3b}$  & $w_{3b}$  & $w_{3b}$ & $w_{3b}$\\
(3d) & \multicolumn{2}{l}{PROMPT-CDSI\textsubscript{d2q}} & $w_{3b}$ & $w_{3b}$  & $w_{3b}$  & $w_{3b}$  & $w_{3b}$ & $w_{3b}$  & $w_{3b}$  & $w_{3b}$ & $w_{3b}$\\
(3e) & Hybrid(DSI-XL, Baseline) \\
\bottomrule
\end{tabular}
}
\vspace{0.25cm}
\caption{Results on the subsets of the XL model on subsets of MS MARCO V1 passage collection.}
\label{table:v1:passage_subset_xl}
\end{table*}

==> tab_nq.tex <==
\begin{table*}[!t]
    \centering
   \caption{DSI results on DPR NQ.
    }
    \resizebox{0.92\textwidth}{!}{
    \begin{tabular}{r|c||cccc||cc|cc|cc}
    \toprule
    \midrule
\bottomrule

    \end{tabular}}
    \label{tab.nq}
\end{table*}

